A High Order Stabilized Solver for the Volume Averaged Navier-Stokes Equations

The Volume-Averaged Navier-Stokes equations are used to study fluid flow in the presence of fixed or moving solids such as packed or fluidized beds. We develop a high-order finite element solver using both forms A and B of these equations. We introduce tailored stabilization techniques to prevent oscillations in regions of sharp gradients, to relax the Ladyzhenskaya-Babuska-Brezzi inf-sup condition, and to enhance the local mass conservation and the robustness of the formulation. We calculate the void fraction using the Particle Centroid Method. Using different drag models, we calculate the drag force exerted by the solids on the fluid. We implement the method of manufactured solution to verify our solver. We demonstrate that the model preserves the order of convergence of the underlying finite element discretization. Finally, we simulate gas flow through a randomly packed bed and study the pressure drop and mass conservation properties to validate our model.

==> nomenclature.tex <==
%***************************
% Nomenclature
%***************************

\makenomenclature
\renewcommand\nomgroup[1]{%
  \item[\itshape \bfseries
  \ifstrequal{#1}{G}{Greek Symbols}{%
  \ifstrequal{#1}{S}{Subscripts}{%
  \ifstrequal{#1}{A}{Abbreviations}{}}}%
]}

\mbox{}

\nomenclature[]{\(\epsilon\)}{void fraction}
\nomenclature[]{\(\bm{u}\)}{velocity}
\nomenclature[]{\(\mathit{m'}\)}{mass source term}
\nomenclature[]{\(\rho\)}{density}
\nomenclature[]{\(p\)}{pressure}
\nomenclature[]{\(\tau\)}{viscous stress tensor}
\nomenclature[]{\(\bm{f}\)}{body forces}
\nomenclature[]{\(F_{pf}\)}{particle fluid forces}
\nomenclature[]{\(\mu\)}{viscosity}
\nomenclature[]{\(\nu\)}{kinematic viscosity}
\nomenclature[]{\(\bm{I}\)}{identity matrix}
\nomenclature[]{\(\Omega\)}{finite element domain}
\nomenclature[]{\(V_{\Omega}\)}{volume of domain $\Omega$}
\nomenclature[]{\(\tau_u\)}{stabilizing parameter}
\nomenclature[]{\(\bm{q}\)}{pressure test function}
\nomenclature[]{\(\bm{v}\)}{velocity test function}
\nomenclature[]{\(\Delta t\)}{time step}
\nomenclature[]{\(h_{conv}\)}{element size related to convection transport}
\nomenclature[]{\(h_{diff}\)}{element size related to diffusion mechanism}
\nomenclature[]{\(\gamma\)}{augmented lagrangian formulation parameter}
\nomenclature[]{\(\varphi\)}{void fraction shape function}
\nomenclature[]{\(L\)}{smoothing length}
\nomenclature[]{\(F_D\)}{drag force}
\nomenclature[]{\(\beta\)}{inter-phase momentum transfer coefficient}
\nomenclature[]{\(np\)}{total number of particles}
\nomenclature[]{\(C_D\)}{drag coefficient}
\nomenclature[]{\(Re\)}{Reynold number}
\nomenclature[]{\(d\)}{diamter}
\nomenclature[]{\(\bm{G}\)}{momentum source term}
\nomenclature[]{\(\norme{E}_2\)}{$\mathcal{L}^2$ norm of the error}
\nomenclature[]{\(e\)}{error at each discretization point}
\nomenclature[]{\(U_{mf}\)}{minimum fluidization velocity}
\nomenclature[]{\(g\)}{gravitational force}
\nomenclature[]{\(\phi\)}{sphericity}
\nomenclature[]{\(\Delta p\)}{pressure drop in bed}
\nomenclature[]{\(Q-Q\)}{velocity-pressure finite element degree}

\nomenclature[S]{\(f\)}{fluid}
\nomenclature[S]{\(p\)}{particle}
\nomenclature[S]{\(k\)}{number of finite elements in domain}
\nomenclature[S]{\(ref\)}{reference}
\nomenclature[S]{\(q\)}{quadrature point}
\nomenclature[S]{\(avg\)}{average value}
\nomenclature[S]{\(b\)}{packed bed}

\nomenclature[A]{\(\mathcal{SR}\)}{strong residual}
\nomenclature[A]{\(VANS\)}{volume averaged Novier Stokes}
\nomenclature[A]{\(SUPG\)}{streamline-upwind Petrove-Galerkin}
\nomenclature[A]{\(PSPG\)}{pressure stabilizing Petrove-Galerkin}
\nomenclature[A]{\(LBB\)}{Ladyzhenskaya–Babuska–Brezzi}
\nomenclature[A]{\(PCM\)}{particle centroid method}
\nomenclature[A]{\(MMS\)}{method of manufactured solutions}
\nomenclature[A]{\(FEM\)}{finite element method}
\nomenclature[A]{\(CFD\)}{computational fluid dynamics}
\nomenclature[A]{\(TFM\)}{two fluid model}
\nomenclature[A]{\(DOF\)}{degrees of freedom}
\nomenclature[A]{\(BDF\)}{backward difference formulation}
\nomenclature[A]{\(DEM\)}{discrete element method}


\begin{small}
\printnomenclature
\end{small}

